Model Theory of Johnson Graphs

A \emph{Johnson graph} $J(n,k)$ is a graph whose vertices are the $k$-element subsets of an underlying set of size $n$ where two vertices are adjacent if they intersect in a subset of size $k-1$. We extend the definition to allow infinite parameters and we study a natural limit theory $T_{\mathcal{J}}$ of Johnson graphs. We show that $T_{\mathcal{J}}$ is complete and we give an axiomatisation of $T_{\mathcal{J}}$, from which we obtain a complete description of the models of $T_{\mathcal{J}}$. We use this to show tameness properties of $T_{\mathcal{J}}$, namely that $T_{\mathcal{J}}$ is $\omega$-stable of Morley rank $\omega$, but not monadically dependent. In particular it follows that the class of all finite Johnson graphs is stable, and therefore dependent but not monadically dependent.

==> Definitions/Ball.tex <==
\begin{definition}
Let $v$ be a vertex in a graph $G$. We call the set of all vertices of distance at most $r$ from $v$  the \emph{ball of radius $r$ around $v$}.
\end{definition}
Observe that $v$ is at distance $0$ from itself and thus included in all balls around $v$.


==> Definitions/Binom.tex <==
\begin{definition}
Let $X$ be a set  and $n$ an integer such that $n≤|X|$.
Then $\binom{X}{n}$ denotes set of all $n$-element subsets of $X$.
\end{definition}


==> Definitions/Neighbourhood.tex <==
\begin{definition}
Let $v$ be a vertex in a graph $G$.
We call the set of all vertices adjacent to $v$  the \emph{neighbourhood of $v$}, denoted $N(v)$.
\end{definition}
Note that
 since we do not allow loops on  vertices we have $v∉N(V)$, and
 what we call here neighbourhood is also sometimes called the \emph{open neighbourhood} around $v$.


==> Definitions/TJ.tex <==
\begin{definition}
	Let $T_\Johnson$ be the set of sentences $σ$ such that for infinite cardinals $κ≥λ$ we have that $J(κ,λ)\models σ$.
\end{definition}


==> EF.tex <==
We will use a type of argument from finite model theory known as Ehrenfeucht-Fraïssé games.
Ehrenfeucht-Fraïssé game arguments are a way to determine if a concept is expressible in first order logic, or if two structures satisfy the same sentences.

The game is played between two players, usually named Spoiler and Duplicator.


\begin{definition}
	Let $L$ be a language with no function symbols, $n∈ℕ$, and  $M$ and $M'$ be $L$-models.
	The \emph{Ehrenfeucht-Fraïssé game} $EF_n(M,M')$ is a $2$ player game played in following way.
	
	In each round first Spoiler plays one element from either $M$ or $M'$, then Duplicator plays one element from whichever model Spoiler did not play in.
	We call the element played in $M$ on the $i$-th round $a_i$ and the element played in $M'$ we call $b_i$ regardless of which player plays them.
	After $n$ rounds have been played we have $(a_i)_{i=1}^n$ and $(b_i)_{i=1}^n$.

	Duplicator has won if for any atomic $L$-formula $ϕ$ and any sequence $(i_j)_{j=1}^k$ with $k≤n$ we have
	$M \models ϕ((a_{i_j})_{j=1}^k) \Leftrightarrow M'\models ϕ((b_{i_j})_{j=1}^k)$, 
	otherwise Spoiler has won.
		 
\end{definition}

Ehrenfeucht-Fraïssé games are a finite analogue to so called back and forth arguments common in model theory.



%To set up the game we choose a game length $n∈ℕ$ and two  $L$-models $M$ and $M'$, and we call this game $EF_n(M,M')$.
%	The game is played for $n$ rounds. 
%	In each round first Spoiler plays one element from either $M$ or $M'$, then Duplicator plays one element from whichever model Spoiler did not play in.
%	We call the element played in $M$ on the $i$-th round $a_i$ and the element played in $M'$ we call $b_i$ regardless of which player plays them.
%	After $n$ rounds have been played we have $(a_i)_{i=1}^n$ and $(b_i)_{i=1}^n$.
%	%Spoiler wins if there exists an atomic $L$-formula $ϕ$ and a sequence  $(i_j)_{j=1}^k$ such that 
%	Duplicator has won if for any atomic $L$-formula $ϕ$ and any sequence $(i_j)_{j=1}^k$ we have
%	$M \models ϕ((a_{i_j})_{j=1}^k) \Leftrightarrow M'\models ϕ((b_{i_j})_{j=1}^k)$, 
%	otherwise Spoiler has won.

Ehrenfeucht and Fraïssé showed that:
	\begin{theorem}[Ehrenfeucht-Fraïssé {\cite[2 and 3]{Ehrenfeucht1961}}]%%%Theorem 2 and 3
		\label{EF}
		If Duplicator has a winning strategy in $EF_n(M,M')$ then for all $L$-sentences $ϕ$ of quantifier depth at most $n$, 
		$M\models ϕ \Leftrightarrow M'\models ϕ$.
	\end{theorem}



We note that if Duplicator has a winning strategy in $EF_n(M,M')$  for all $n∈ℕ$ that means that the models $M$ and $M'$ are indistinguishable from the perspective of first order logic.
This means that any characteristic that $M$ has and $M'$ does not have  cannot be expressed in first order logic.

\begin{example}
	Connectivity in graphs is not first order expressible.
	See \cite[3.19]{LibkinBook} for details.
%	Show that connectedness is not expressible in first order logic, can use corollary 3.19 in libkins book.
\end{example}


==> Theorems/Transfinite.tex <==
\begin{theorem}
\label{InfiniteEF}
Let $(κ_i)_{i∈I}$ and $(λ_i)_{i∈I}$ be families of infinite cardinals.
Duplicator has a winning strategy in  the Ehrenfeucht-Fraïssé game
$EF_{\floor{\log{t}}}(J(n,k),\bigsqcup_{i∈I} J'(κ_i,λ_i))$
where $t=\floor{\frac{\min(k,n-k)}{2}}$.
\begin{proof}
Duplicator's strategy is more or less identical to the one he uses in the proof of Theorem \ref{ThmEF}. %$EF_{\log{t}}(J(n,k),J(n',k'))$.

It is worth noting that for the purposes of that strategy there is no difference between two vertices in $\bigsqcup J'(κ_i,λ_i)$ being in
different connected components and merely being further than distance $\frac{t}{2^m}$ apart.
Thus the following proof is similar to what we have already presented.

Since $J(n,k)\cong J(n,n-k)$ we can assume without loss  of generality $n≥2k$.
This means that $t=\floor{\frac{k}{2}}$.

As a clarification on notation	we will call the vertex played on turn $i$ in $J(n,k)$, $a_i$ regardless of which player plays it.
Likewise 			we will call the vertex played on turn $i$ in $\bigsqcup_{j∈I} J'(κ_j,λ_j)$, $b_i$ regardless of which player plays it.

Without loss of generality we can assume that each of the graphs $J'(κ_i,λ_i),i∈I$ have underlying  sets  $Y_i,i∈I$ that are pairwise disjoint.
	We call their union $⋃_{i∈I}Y_i=Y$.
Duplicator will be building up a partial bijection $f$ from $X$, the underlying set of $J(n,k)$, to $Y$.
We do this by creating a sequence $(f_i)_{i=1}^{\floor{\log{t}}}$ where $f_1$ is the empty map, $f_{\floor{\log{t}}}=f$ and  $f_{i+1}$ extends $f_{i}$.
%It is through this sequence of functions that duplicator is able to avoid any traps set by spoiler and is guaranteed a move on every turn of the game.

Now we are ready to play the game.
\paragraph{Base case:}

By vertex transitivity, the first move of the game is arbitrary both by spoiler and duplicator.

Duplicator sets $f_1$ to be the empty map.

For the second move
if spoiler plays $a_2$ duplicator starts by looking at $a_1\symdiff a_2$.
If $|a_1\symdiff a_2|≤t$ then duplicator plays a $b_2$ such that $|a_1\symdiff a_2|=|b_1\symdiff b_2|$ then duplicator forms a bijection $f_2$ from $a_1\symdiff a_2$ to $ b_1\symdiff b_2$
such that $x∈a_1\iff f_{2}(x)∈b_1$ and  $x∈a_2\iff f_{2}(x)∈b_2$.
If $|a_1\symdiff a_2|>t$ then duplicator plays a $b_2$ such that $\min(|a_1\symdiff a_2|,2t)=|b_1\symdiff b_2|$ and sets $f_2=f_1$ to be the empty map.

%%%%%%%%%%%%
\paragraph{Induction hypothesis:}

After $m-1$ moves by both players which grant us the sequences, $(a_i)_{i=1}^{m-1}, (b_i)_{i=1}^{m-1}$ in $J(n,k)$ and $\bigsqcup_{i∈I} J'(κ_i,λ_i)$ respectively  duplicator has formed the function
$f_{m-1}$ in such a way that if
$|a_i\symdiff a_j|≤\frac{t}{2^{m-1}}$ or $|b_i\symdiff b_j|≤\frac{t}{2^{m-1}}$  then % $a_i\symdiff a_j ⊆ dom(f_{m-1}$.
$a_i\symdiff a_j⊆ \dom(f_{m-1})$, $b_i \symdiff b_j ⊆ \img(f_{m-1})$ and
$$x∈a_i∖ a_j \iff f_{m-1}(x)∈b_i∖ b_j$$
Note that this implicitly means that for all $i,j<m$ if $d(a_i,a_j)≤ \frac{t}{2^m}$ or $d(b_i,b_j)≤\frac{t}{2^m}$ then  $d(a_i,a_j)=d(b_i,b_j)$.

%%%%%%%%%%%%
\paragraph{Inductive step:}

\paragraph{Assume spoiler plays $a_m$.} % duplicator looks at those $i<m$ such that $d(a_i,a_m)<\frac{t}{2^m}$.
Let $M⊆[1,m-1]∩ℕ$ be such that $i∈M$ if and only if $d(a_i,a_m)≤\frac{t}{2^m}$.
%
If $M=∅$ then duplicator sets $f_m=f_{m-1}$ and plays a $b_m$ such that $d(b_i,b_m)>\frac{t}{2^m}$ for all $i<m$.
Such a vertex always exists since each connected component of $\bigsqcup_{i∈I} J'(κ_i,λ_i)$ has infinite diameter.
%Such a vertex always exists due to Lemma \ref{NoCover}.

Assume $M≠∅$.
For every $i,j∈M$ we have that $d(a_i,a_j)≤ \frac{2t}{2^{m}}$ so by induction hypothesis $a_i\symdiff a_j⊆ \dom(f_{m-1})$.
Note that by our induction hypothesis, for all $i,j∈M$ we have that  $d(b_i,b_j)$ is finite and thus $b_i$ and $b_j$ are in the same connected component.
Without loss of generality assume it is the $y$-th component.
Duplicator has to extend $f_{m-1}$ to $f_m$ with domain
$$\dom(f_{m-1})∪⋃_{i∈M} a_m\symdiff a_i$$  in such a way that if $x∈a_i∩ \dom(f_{m})$ then $f_{m}(x)∈b_i$ and every element in $( a_m∖(⋃_{i<m}a_i) )∩ \dom(f_m)$
	gets mapped to an element that is in $Y_y ∖ ⋃_{i∈M}b_i$.

$$(⋃_{i∈M} a_m\symdiff a_i) ∖ \dom(f_{m-1})  ⊆  (a_m ∖ ⋃_{i∈M}a_i) ∪ ((⋂_{i∈M}a_i)∖a_m)$$
that is to say, every element that duplicator is adding to  the domain of $f_m$ is either in only $a_m$  or in every other $a_i$ for $i∈M$.
%%for any $i,j∈M$ that $d(a_i,a_j)≤ 2 \frac{t}{2^m}=\frac{t}{2^{m-1}}$ so any element in $a_i\symdiff a_j$ will by our construction be in the domain of $f_{m-1}$.
So the elements in the domain of $f_m$ that aren't in the domain of $f_{m-1}$ will be in either
$(⋂_{i∈M} a_i) ∖ a_m$
or
$a_m∖⋃_{i∈M} a_i$
and thus need to be mapped to
$⋂_{i∈M} b_i$
and
$Y_y∖(⋃_{i∈M} b_i)$ respectively.
In each case we need to show that the domain contains at most as many elements as the image.


\paragraph{Case 1:}
Mapping
$(⋂_{i∈M} a_i) ∖ a_m$
to
$(⋂_{i∈M} b_i)$
is possible since:
We know that for all $i∈M$ $|a_i∖a_m|≤ \frac{t}{2^m}$ so we get
$$|(⋂_{i∈M} a_i) ∖ a_m| ≤ \frac{t}{2^m} ≤  t$$
and
%Since for all $i,j∈M$ we have $d(a_i,a_j)=d(b_i,b_j)$ we get that
%$$|(⋂_{i∈M} b_i)|≥ k- \frac{|M|t}{2^m} ≥ k - \frac{tm}{2^m} ≥ k - t ≥ t$$
$$|(⋂_{i∈M} b_i)|= λ ≤ t$$

\paragraph{Case 2:}
Mapping
$a_m∖⋃_{i∈M} a_i$
to
$Y_y∖(⋃_{i∈M} b_i)$.

Since for $i∈M$ $|a_m∖a_i|≤ \frac{t}{2^m}$ we get
$$|a_m∖⋃_{i∈M} a_i| ≤ \frac{t}{2^m}≤ t$$ %% this bound is acheived by all members of M splitting off the same elements of a_m
and
since
%$$|Y∖(⋃_{i∈M} b_i)| ≥  n - (k + |M|\frac{t}{2^m}) ≥ (n - k) - m\frac{t}{2^m} ≥ k - \frac{mt}{2^m} ≥ k-t ≥ t$$
$$|Y_y∖(⋃_{i∈M} b_i)| =  κ  ≥ t$$

Duplicator then plays $b_m=f_m[a_m∩ \dom(f_m)] ∪ ⋂_{i∈M}b_i$.
By our definition of $f_m$, and the fact that $|⋂_{i∈M}b_i|$ we get that $b_m$ is in fact a  vertex.
Note that then we have for all $i∈M$ $d(a_m,a_i)=d(b_m,b_i)$.
So by induction hypothesis  we have for $i,j≤m$  that if
$|a_i\symdiff a_j|≤\frac{t}{2^{m}}$ or $|b_i\symdiff b_j|≤\frac{t}{2^{m}}$  then
$a_i\symdiff a_j⊆ \dom(f_{m})$ , $b_i \symdiff b_j ⊆ \img(f_{m})$ and
$$x∈a_i∖ a_j \iff f_{m}(x)∈b_i∖ b_j$$

\paragraph{Assume spoiler plays  $b_m$.}

Let $M⊆[1,m-1]∩ℕ$ be such that $i∈M$ if and only if $d(b_i,b_m)≤\frac{t}{2^m}$.

If $M=∅$ then duplicator sets $f_m=f_{m-1}$ and plays an $a_m$ such that $d(a_i,a_m)>\frac{t}{2^m}$ for all $i<m$.
Such a vertex always exists due to Lemma \ref{NoCover}.

Assume $M≠∅$.
Duplicator then extends $f_{m-1}$ to $f_m$ with image
%$$dom(g_{m-1})∪⋃_{i∈M} g_m\symdiff g_i$$  in such a way that if $x∈b_i$ then $g_{m}(x)∈a_i$ and every element in $b_m∖(⋃_{i<m}b_i)$
$$\img(f_{m-1})∪⋃_{i∈M} b_m\symdiff b_i$$  in such a way that if $x∈a_i$ then $f_{m}(x)∈b_i$ and every element in $b_m∖(⋃_{i<m}b_i)$
	gets mapped to by an element that is  in the  complement  of $⋃_{i<m}a_i$.


In this case the elements in the image of $f_m$ that aren't in the image of $f_{m-1}$ will be in either
$(⋂_{i∈M} b_i) ∖ b_m$
or
$b_m∖⋃_{i∈M} b_i$
and thus need to be mapped onto by
$(⋂_{i∈M} a_i)$
and
$X∖(⋃_{i∈M} a_i)$ respectively.
In each case we need to show that the image contains at most as many elements as the domain.


\paragraph{Case 1:}
Mapping
$(⋂_{i∈M} a_i)$
to
$(⋂_{i∈M} b_i) ∖ b_m$
is possible since:
$$|(⋂_{i∈M} b_i) ∖ b_m| ≤ \frac{t}{2^m} ≤  t$$
and
$$|(⋂_{i∈M} a_i)|≥ k- \frac{|M|t}{2^m} ≥ k - \frac{tm}{2^m} ≥ k - t ≥ t$$

\paragraph{Case 2:}
Mapping
$X∖(⋃_{i∈M} a_i)$
to
$b_m∖⋃_{i∈M} b_i$
is possible since
$$|b_m∖⋃_{i∈M} b_i| ≤ \frac{t}{2^m}≤ t$$
and
$$|X∖(⋃_{i∈M} a_i)| ≥ n-(k+|M|\frac{t}{2^m})= (n-k) - m\frac{t}{2^m}≥k-t\frac{m}{2^m}≥k-t≥t$$



By our definition of $f_m$, we get $f_m^{-1}[b_m ∩ \img(f_m)]$ has size $k-|⋂_{i∈M}a_i|$.
Duplicator then plays $a_m=f_m^{-1}[b_m∩ \img(f_m)] ∪ ⋂_{i∈M}a_i$.
Note that then we have for all $i∈M$ $d(a_m,a_i)=d(b_m,b_i)$.
So by induction hypothesis  we have for $i,j≤m$ that if
$|a_i\symdiff a_j|≤\frac{t}{2^{m}}$ or $|b_i\symdiff b_j|≤\frac{t}{2^{m}}$  then
$a_i\symdiff a_j⊆ \dom(f_{m})$ , $b_i \symdiff b_j ⊆ \img(f_{m})$ and
$$x∈a_i∖ a_j \iff f_{m}(x)∈b_i∖ b_j$$


So after $m$ moves by both players, duplicator has formed the function $f_{m}$ in such a way that if
$|a_i\symdiff a_j|≤\frac{t}{2^{m}}$  then  $x∈a_i ∖ a_j \iff f_m(x)∈b_i∖b_j$ and $x∈a_j∖a_i \iff f_{m}(x)∈ B_J∖B_I$. %\symdiff a_j \implies f_{m}(x)∈b_i\symdiff b_j$.
This concludes the inductive step.

At the end of the game we have for any $i,j≤\floor{\log{t}}$
that if
$d(a_i,a_j)≤\floor{\frac{t}{2^{\log{t}}}}=1$ or
$d(b_i,b_j)≤\frac{t}{2^{\log{t}}}=1$
then
$d(a_i,a_j)=d(b_i,b_j)$.
In particular this means that $Ea_ia_j$ if and only if $Eb_ib_j$ so the substructures
$A=\{a_i|1≤i≤\log(t)\}$ in $J(n,k)$
and
$B=\{b_i|1≤i≤\log(t)\}$ in $\bigsqcup_{i∈I} J'(κ_i,λ_i)$ are isomorphic.
\end{proof}
\end{theorem}

